Second order semi-parametric inference for multivariate log Gaussian Cox processes

This paper introduces a new approach to inferring the second order properties of a multivariate log Gaussian Cox process (LGCP) with a complex intensity function. We assume a semi-parametric model for the multivariate intensity function containing an unspecified complex factor common to all types of points. Given this model we exploit the availability of several types of points to construct a second-order conditional composite likelihood to infer the pair correlation and cross pair correlation functions of the LGCP. Crucially this likelihood does not depend on the unspecified part of the intensity function. We also introduce a cross validation method for model selection and an algorithm for regularized inference that can be used to obtain sparse models for cross pair correlation functions. The methodology is applied to simulated data as well as data examples from microscopy and criminology. This shows how the new approach outperforms existing alternatives where the intensity functions are estimated non-parametrically.

==> bib/litteratur.tex <==
\chapter{Litteratur} \nonumber

Møller, J. \& Waagepetersen, R. P. (2004). $Statistical$ $Inference$ $and$ $Simulation$ $for$ $Spatial$ $Point$ $Processes$. Chapman \& Hall/CRC. 1. udgave.
\\

\noindent van Lieshout, M. (2010). $Spatial$ $Point$ $Process$ $Theory$. Handbook of Spatial Statistics. CRC Press, 263-282.









==> sections/conclusion.tex <==
\section{Conclusion} \label{sec:con}

==> sections/dataexample.tex <==
\section{Data example} \label{sec:dataanalysis}
\subsection{Lymph node metastasis}
Figure \ref{fig:data}  shows a slice of a lymph node metastasis. Using machine learning techniques for segregation the lymph node metastasis slice can be recognized as a four-variate point pattern data. The four types of points are: 1) Hypoxic tumor cells (Hypoxic), 2) Normoxic tumor cells (Normoxic), 3) Stroma cells (Stroma) and 4) Cytotoxic T-lymphocytes (CD8). 
\begin{figure}[ht!]
\centering
\begin{tabular}{cc}
\includegraphics[scale=0.094]{figures/data_analysis/lymph_metastasis/original_data.jpg}
\includegraphics[scale=0.30]{figures/data_analysis/lymph_metastasis/thinbivar_new.png}
\end{tabular}
\caption{Left: Fluorenscense channels in lymph node metastasis. Right: Independent thinned bivariate point pattern of Stroma (red) and CD8 (yellow).} \label{fig:data}
\end{figure}

We analyze the bivariate point pattern that consists of 6015 Stroma points and 1466 CD8 points, while we exclude the Hypoxic points and the Normoxic points. Oncologists among other could be interested in the second order properties within and between Stroma and CD8 cells. We study the bivariate second order property by assuming that Stroma and CD8 can be modeled by a bivariate LGCP and estimate the parameter vector $\btheta$ using the second order MLL. Since the PCF is invariant under independent thinning of a point process, we can do independent thinning of Stroma and CD8 and expect the same conclusion when analyzing the second order properties of the bivariate point pattern. We independently thin Stroma and CD8 by independently remove $50\%$ of the points in each pattern. There are no spatial covariates available, thus we only estimate the intercept between Stroma and CD8. Following \cite{hessellund} we choose CD8 as the baseline and estimate $\bbeta=(\beta_{\textup{stroma}},\beta_{\textup{CD8}})^T=(\gamma_{\textup{stroma}}-\gamma_{\textup{CD8}},\gamma_{\textup{CD8}}-\gamma_{\textup{CD8}})^T$ by $\hat{\beta}_{\textup{stroma}}= \textup{log} (3007/733)=1.41$ and $\hat{\beta}_{\textup{CD8}}=0$. Due to our data is bivariate, we only consider $q=1$ and choose $\lambda$ using a $10$-fold CV as described in Section \ref{sec:cvlambda}, where we resample $25$ times. We choose $\lambda$ among the sequence:
\begin{align*}
\boldsymbol{\lambda}=(100,90,80,70,60,50,40,30,20,15,10,8,5,2,1,0)
\end{align*}
We choose the maximal distance between pairs of points to be $400$, which is determined by looking at the size of the observation window. 

\begin{figure}[ht!]
\centering
\begin{tabular}{c c c}
\includegraphics[scale=0.3]{figures/data_analysis/lymph_metastasis/2020-05-27/mean_cv.pdf}
\includegraphics[scale=0.3]{figures/data_analysis/lymph_metastasis/2020-05-27/pcfs.pdf}
\includegraphics[scale=0.3]{figures/data_analysis/lymph_metastasis/2020-05-27/cross_pcf.pdf}
\end{tabular}
\caption{Left: Mean CV-score for $\boldsymbol{\lambda}$ and $q=1$. Middle: Plot of PCF's and cross-PCF using $\lambda=0$ and $q=1$. Right: Plot of PCF ratio and cross-PCF ratio using $\lambda=0$ and $q=1$.} \label{fig:lymphplot}
\end{figure}

According to left panel in Figure \ref{fig:lymphplot} we choose $\lambda=0$. Thus we do not penalize $\balpha$ in our data analysis. Our estimates in Figure \ref{fig:lymphresult} is generated through a series of warm starts using $\boldsymbol{\lambda}$.
\begin{figure}[ht!]
\centering
\begin{tabular}{| c | c  c  c  c|}
\hline
& $\hat{\balpha}$ & $\hat{\xi}$ & $\hat{\bsigma}^2$& $\hat{\bphi}$ \\
\hline
Stroma & 0.34 & 79 & 0.56 & 82.3 \\
CD8 & 0.47 & 79 & 1.22 & 116.7\\
  \hline
\end{tabular} 
\caption{Table of parameter estimates for Stroma and CD8.} \label{fig:lymphresult}
\end{figure}

Based on the estimated parameters in Figure \ref{fig:lymphresult} we conclude that Stroma and CB8 is positively correlated. Notice, that CB8 is also estimated to be more clustered than Stroma, which is illustrated in the middle panel in Figure \ref{fig:lymphplot}. As a brief validation of the estimated model, we can compare ratios of fitted PCFs or cross-PCFs to a corresponding non-parametric estimate developed in \cite{hessellund}. In this example, we choose $g_{St,St}(r)/g_{CD8,CD8}(r)$ and $g_{St,CD8}(r)/g_{CD8,CD8}(r)$ as the PCF ratio and cross-PCF ratio to validate our fitted parametric model from. Following right panel in Figure \ref{fig:lymphplot} the fitted paramatric PCF ratio and cross-PCF ratio has the same trend as the corresponding non-parametric estimate. Thus, the fitted parameters seems reliable based on the comparison of the parametric and non-parametric estimate of the PCF ratio and cross-PCF ratio. 

\subsection{Washington DC street crimes}
 
\begin{figure}[ht!]
\centering
\begin{tabular}{| c | c  c  c  c |}
\hline
Crime type & $\hat{\alpha}$ & $\hat{\xi}$ &  $\hat{\sigma}^2$  & $\hat{\phi}$   \\
\hline
Other theft & 0.29 & 0.87 & 0.29 & 0.87 \\
Burglary  & 0.29 & 0.87 & 0.29 & 0.87  \\
Assault & 0.29 & 0.87 & 0.29 & 0.87  \\
Vehicle Theft & 0.29 & 0.87 & 0.29 & 0.87   \\
Theft F. Auto & 0.29 & 0.87 & 0.29 & 0.87\\
Robbery & 0.29 & 0.87 & 0.29 & 0.87 \\
  \hline
\end{tabular} 
\end{figure}

\begin{figure}[ht!]
\centering
\begin{subfigure}{0.32\textwidth}
\includegraphics[scale=0.3]{figures/data_analysis/crime/2020-05-26/pcf.pdf}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[scale=0.3]{figures/data_analysis/crime/2020-05-26/gx1.pdf}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[scale=0.3]{figures/data_analysis/crime/2020-05-26/gx2.pdf} 
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[scale=0.3]{figures/data_analysis/crime/2020-05-26/gx3.pdf}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[scale=0.3]{figures/data_analysis/crime/2020-05-26/gx4.pdf}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\includegraphics[scale=0.3]{figures/data_analysis/crime/2020-05-26/gx5.pdf}
\end{subfigure}
\end{figure}


\begin{figure}[ht!]
\centering
\begin{subfigure}{0.5\textwidth}
\includegraphics[scale=0.5]{figures/data_analysis/crime/2020-05-26/PCF_ratio.pdf}
\end{subfigure}
\end{figure}

% The initial parameters is given by
%boxplot of CV score over 100 resamples

==> sections/estimation.tex <==
\section{Second order multinomial logistic regression} \label{sec:esti}
To obtain an estimate of the parameter vector $\btheta=(\btheta_1,\dots,\btheta_p) \in \R^{d}$, where $d=(p+1)q+2p$ we consider a  second order conditional composite likelihood (CCL) approach. Since the estimation procedure in \cite{hessellund} provides consistent estimates of $\bbeta_i$, for $i=1,\dots,p-1$, we only focus on the parameter vector $\btheta$. Thus, we suppress the function arguments $\hat{\bbeta}$ in the rest of this paper and denote by $\hat{f}_i(\bu)=\textup{exp}(\hat{\bbeta}_i^T \bz(\bu))$. The idea is to generate probabilities for a random pair of points, say $(\bu,\bv)$, to be from point process $X_i$ and $X_j$. We do that by defining the following second order conditional probabilities: 
\begin{align} \label{eq:proba}
\textup{p}_{ij}(\bu,\bv; \btheta) = \frac{\rho_{ij}(\bu,\bv;\btheta_{ij})}{\sum_{k \leq l} \rho_{kl}(\bu,\bv;\btheta_{kl})} = \frac{\hat{f}_i(\bu) \hat{f}_j(\bv) g_{ij}(\bu,\bv; \btheta_{ij})}{\sum_{k \leq l} \hat{f}_k(\bu) \hat{f}_l(\bv) g_{kl}(\bu,\bv; \btheta_{kl})},
\end{align} 
where $\rho_0(\bu)\rho_0(\bv)$ cancels out in \eqref{eq:proba}, hence the probabilities do not depend on $\rho_0(\cdot)$. Furthermore, we define a second order multinomial logistic likelihood (MLL) function by:
\begin{align} \label{eq:lik}
L(\btheta)= \prod_{i \leq j} \prod_{\substack{\bu \in X_i \cap W \\ \bv \in X_j \cap W \\ ||\bu-\bv|| \leq R}}^{\neq} \textup{p}_{ij}(\bu,\bv; \btheta),
\end{align}
where $R \geq 0$. Notice that the constraint $||\bu-\bv|| \leq R$ reduces the computation time, but $R$ should still be chosen such that $g_{ij}(\bu,\bv) \approx 1$ for all $\bu,\bv$ with $||\bu-\bv||>R$. The second order MLL function \eqref{eq:lik} has some resembles to a multinomial logistic regression likelihood function (of first order). However, in contrast to first order multinomial logistic regression problems we do not need to reparameterize each $\btheta_{ij}$ by choosing one parameter vector, say $\btheta_{mn}$, as a baseline in order to make each $\btheta_{ij}$ identifiable. This is simply avoided due to the construction of the likelihood with $p^2$ probabilities $\textup{p}_{ij}(\bu,\bv;\btheta)$ for $\btheta$, which contains $p$ independent parameter vectors $\btheta_i$. The second order log-MLL function $l(\btheta)=\textup{log}(L(\btheta))$ is then:
\begin{align} \label{eq:loglik}
l(\btheta)=\sum_{i \leq j} \sum_{\substack{\bu \in X_i \cap W \\ \bv \in X_j \cap W \\ ||\bu- \bv|| \leq R}}^{\neq} \textup{log}\left(\rho_{ij}(\bu,\bv;\btheta_{ij}) \right) -  \textup{log}\left( \sum_{k \leq l} \rho_{kl}(\bu,\bv;\btheta_{kl}) \right),
\end{align}
which is the object function that we want to maximize with repect to $\btheta$. Instead we turn \eqref{eq:loglik} into a minimization problem and consider the negated second order log-MLL, denote by $l_-(\btheta) = - l(\btheta)$, which we minimize with respect to $\btheta$. 

\subsection{Cyclic coordinate descent algorithm}
For the rest of this paper we consider $\btheta$ in terms of regularized and non-regularized parameters. We aim to regularize the cross-dependence parameters $\balpha$, while $\bpsi=(\bxi,\bsigma^2,\bphi)^T$ is the parameter vector with no regularization. Thus, the estimation of $\balpha$ is treated seperately from $\bpsi$. In order to minimize $l_-(\btheta)$ with respect to $\btheta$, we consider a cyclic coordinate descent algorithm. Denote by $\btheta^{(n)}=(\balpha^{(n)},\bpsi^{(n)})^T$ the current value of $\btheta$. For given values of $\bpsi^{(n)}$ we estimate $\balpha$ by considering the following regularized log-MLL:  
\begin{align} \label{eq:penalize}
Q_{\lambda}(\balpha,\bpsi^{(n)}) = l_-(\balpha,\bpsi^{(n)}) + \lambda \sum_{k=1}^p || \balpha_{k} ||,
\end{align} 
where $\lambda \sum_{k=1}^p || \balpha_{k} ||$ is a group lasso that serves to regularize $\balpha$ for a given choice of the tuning parameter $\lambda$. In Section \ref{sec:cvlambda} we propose a cross-validation procedure to choose $\lambda$. By using line search we update $\balpha^{(n+1)}=\balpha^{(n)} + t(\hat{\balpha}-\balpha^{(n)})$ such that $l_-(\balpha^{(n+1)},\bpsi^{(n)}) \leq l_-(\balpha^{(n)},\bpsi^{(n)})$ for some $t>0$. We obtain an estimate of $\balpha$ as the solution to 
\begin{align} \label{eq:argmin1}
\hat{\balpha}&= \textup{arg min}_{\balpha}  Q_{\lambda}(\balpha,\bpsi^{(n)}).
\end{align}
The estimation procedure for \eqref{eq:penalize} is described in details in Section \ref{sec:algo}. For the non-regularized parameter vectors we also apply line search to update $\bpsi^{(n+1)}$ in turn, where we obtain an estimate of each parameter vector as the solution to

\begin{align*}
\hat{\bpsi}&= \textup{arg min}_{\bpsi} l_-(\balpha^{(n+1)}, \bpsi)
\end{align*}
In practice, we estimate $\bxi$, $\bsigma$ and $ \bphi$ using the R command \texttt{optim}. The coordinate descent algorithm is set to converge, whenever
\begin{align*}
\left\vert \frac{l_-(\btheta^{(n+1)})-l_-(\btheta^{(n)})}{l_-(\btheta^{(n)})} \right\vert < \epsilon,
\end{align*}
for some $\epsilon > 0$.

\subsection{Group-regularization using proximal Newton methods} \label{sec:algo}
In connection to first order multinomial logistic regression problems no closed form solutions exist for $\balpha$ using \eqref{eq:loglik}, hence we need to estimate the parameters using iterative procedures. Following \cite{lee} we can minimize \eqref{eq:penalize} with respect to $\balpha$ using proximal Newton methods. Consider a second order Taylor approximation of $l_-(\balpha,\bpsi^{(n)})$ with initial parameters $\balpha^{(n)}$ and $\bpsi^{(n)}$:
\begin{align} \label{eq:taylor}
f(\balpha,\bpsi^{(n)}) & = l_-(\balpha^{(n)},\bpsi^{(n)}) + (\balpha - \balpha^{(n)})^T\best(\balpha^{(n)},\bpsi^{(n)}) \nonumber \\
& + \frac{1}{2}(\balpha - \balpha^{(n)})^T \textup{H} (\balpha^{(n)},\bpsi^{(n)})(\balpha - \balpha^{(n)}),
\end{align} 
where \begin{align} \label{eq:estfct}
\best(\btheta^{(n)})  =\nabla_{\balpha}l_-(\btheta^{(n)})= \sum_{i \leq j} \sum_{\substack{\bu \in X_i \cap W \\ \bv \in X_j \cap W \\ ||\bu -\bv|| \leq R}}^{\neq} \left( \frac{\sum_{k \leq l} \nabla_{\balpha} \rho_{kl}(\bu,\bv;\btheta^{(n)})}{\sum_{k \leq l }  \rho_{kl}(\bu,\bv;\btheta^{(n)})} - \frac{\nabla_{\balpha} \rho_{ij}(\bu,\bv;\btheta^{(n)})}{\rho_{ij}(\bu,\bv;\btheta^{(n)})} \right)
\end{align}
is the estimating function with respect to $\balpha$. Notice that \eqref{eq:estfct} does not depend on $\rho_0(\bu)\rho_0(\bv)$ and following Lemma \ref{lem:unb} $\best(\btheta^*)$ is an unbiased estimating function. Furthermore 
\begin{align} \label{eq:ehess}
\textup{H}(\btheta^{(n)})=\textup{E} [\nabla^2_{\balpha} l_-(\btheta^{(n)})] = \int_{W^2} 1_R(\bu,\bv)\textup{Cov} \left(X(\bu,\bv;\btheta^{(n)}) \right) \sum_{i \leq j} \rho_{ij}(\bu,\bv;\btheta_{ij}^{(n)}) \textup{d} \bu \textup{d} \bv
\end{align}
is the expected hessian with respect to $\balpha$, where $1_R(\bu,\bv)=1[||\bu-\bv \leq R||]$ and $X(\bu,\bv;\btheta^{(n)}) $ denote a random vector which takes values $\nabla_{\balpha} \textup{log}(\rho_{ij}(\bu,\bv;\btheta^{(n)}))$ with probability $\textup{p}_{ij}(\bu,\bv;\btheta^{(n)})$, $j=1,\dots, p$ and $i \leq j$. The expression of \eqref{eq:ehess} is derived in Lemma \ref{prop:sens}. We approximate \eqref{eq:ehess} using \eqref{eq:campbell}:
\begin{align*}
\hat{H}(\btheta^{(n)})=\sum_{i \leq j} \sum_{\substack{\bu \in X_i \cap W \\ \bv \in X_j \cap W \\ ||\bu -\bv|| \leq R}}^{\neq} \textup{Cov} \left(X(\bu,\bv;\btheta^{(n)}) \right),
\end{align*}
which is an unbiased estimate of $\textup{H}(\balpha^{(n)},\bpsi^{(n)})$ that does not depend on $\rho_0(\bu)\rho_0(\bv)$. Since $\textup{H}(\balpha^{(n)},\bpsi^{(n)})$ is a symmetric, positive semi-definite $qp \times qp$ matrix, the eigendecomposition implies that $\textup{H}(\balpha^{(n)},\bpsi^{(n)})^{1/2}=UD^{1/2}U^T$, where $D^{1/2}=\textup{diag}(\textup{l}^{1/2})$ for non-negative eigenvalues $\textup{l}_i$, $i = 1, \dots, qp$, and the columns of $U$ correspond to the eigenvectors of $\textup{H}(\balpha^{(n)},\bpsi^{(n)})$. 

Using $f(\balpha,\bpsi^{(n)})$ we can rewrite \eqref{eq:loglik} as a least squares problem. When taking a closer look at \eqref{eq:taylor}, we see that:
\begin{align} \label{eq:minfct1}
\hat{\balpha} \approx &\textup{arg min}_{\balpha} \bigg( f(\balpha,\bpsi^{(n)}) \bigg) \\
 \equiv & \textup{arg min}_{\balpha} \bigg( (\balpha - \balpha^{(n)})^T \best(\balpha^{(n)},\bpsi^{(n)})+ \frac{1}{2}(\balpha - \balpha^{(n)})^T \textup{H} (\balpha^{(n)},\bpsi^{(n)})(\balpha - \balpha^{(n)}) \bigg) \nonumber\\
 \equiv & \textup{arg min}_{\balpha} \bigg( -(\balpha - \balpha^{(n)})^T  \textup{H} (\balpha^{(n)},\bpsi^{(n)})K + \frac{1}{2}(\balpha - \balpha^{(n)})^T \textup{H} (\balpha^{(n)},\bpsi^{(n)})(\balpha - \balpha^{(n)}) \bigg) \nonumber\\
 \equiv & \textup{arg min}_{\balpha} \bigg( \frac{1}{2}(K-(\balpha - \balpha^{(n)}))^T \textup{H} (\balpha^{(n)},\bpsi^{(n)})(K-(\balpha - \balpha^{(n)})) \bigg) \nonumber,
\end{align}
where $K=-\textup{H}^{-1}(\balpha^{(n)},\bpsi^{(n)})\best(\balpha^{(n)},\bpsi^{(n)})$. Hence, we see \eqref{eq:minfct1} is a least squares problem:
\begin{align} \label{eq:minfct2}
\hat{\balpha} \approx & \textup{arg min}_{\balpha} \bigg(\frac{1}{2} ||\textup{H} (\balpha^{(n)},\bpsi^{(n)})^{1/2}(K-(\balpha- \balpha^{(n)}))||^2 \bigg) \nonumber\\
\equiv & \textup{arg min}_{\balpha} \bigg( \frac{1}{2} ||Y -X\balpha ||^2 \bigg) ,
\end{align}
where
\begin{align*}
Y&=\textup{H}(\balpha^{(n)},\bpsi^{(n)})^{1/2}\left( -\textup{H}(\balpha^{(n)},\bpsi^{(n)})^{-1}\best(\balpha^{(n)},\bpsi^{(n)})+\balpha^{(n)} \right) \quad \textup{and} \\
X&=\textup{H}(\balpha^{(n)},\bpsi^{(n)})^{1/2}.
\end{align*}
Our approximate solution to \eqref{eq:argmin1} is then given by:
\begin{align*}
\hat{\balpha} \approx \textup{arg min}_{\balpha} \bigg( \frac{1}{2} ||Y -X\balpha ||^2  + \lambda \sum_{k=1}^p || \balpha_{k} || \bigg).
\end{align*}
In the rest of this paper we will name $\frac{1}{2} ||Y -X\balpha ||^2$ as the $loss$ function. This approach is related to the work by \cite{meier}, who considered group lasso penalization for logistic regression and derived an algorithm by a combination of proximal Newton methods and line search. In order to solve \eqref{eq:minfct2} we apply the so-called $groupwise$-$majorization$-$descent$ (GMD) algorithm proposed by \cite{Yang}, which is a suitable algorithm for e.g. least squares regularization problems. The GMD algorithm is described in details in Section \ref{sec:gdm}.

\subsection{GMD algorithm} \label{sec:gdm}
The GMD algorithm proposed by \cite{Yang} is a group lasso algorithm that is suitable for different classes for regularization problems, including least squares and logistic regression problems. The GMD algorithm is implemented in R as the package \texttt{gglasso}. \cite{Yang} expands the algorithms proposed by \cite{fried1} and \cite{Yuan}, since \cite{Yang} solve group lasso problems with a general design matrix. In contrast, the algorithms proposed by \cite{fried1} and \cite{Yuan} requires a groupwise orthonormal condition for the design matrix. Furthermore, \cite{Yang} shows in case of logistic regularization problems that the GMD algorithm outperforms the algorithm in the R package \texttt{grplasso} proposed by \cite{meier} in terms of computation time.

Denote by $\boldsymbol{D}$ the working data and $\boldsymbol{\pi} \in \R^{d_1}$ the parameter vector of interest with $\boldsymbol{\pi}^*$ as the true value of $\boldsymbol{\pi}$. The GMD algorithm consider group lasso problems for general loss functions $\textup{L}(\boldsymbol{\pi}|\boldsymbol{D})$ that satisfies a certain $quadratic$ $majorization$ (QM) condition:
\begin{enumerate}
\item $\textup{L}(\boldsymbol{\pi}|\boldsymbol{D})$ is everywhere differentiable as a function of $\boldsymbol{\pi}$,

\item \label{it:2} There exists $d_1 \times d_1$ matrix $H$, which only depend on $\boldsymbol{D}$, such that for all $\boldsymbol{\pi}, \boldsymbol{\pi}^*$:
\begin{align*}
\textup{L}(\boldsymbol{\pi}|\boldsymbol{D}) \leq \textup{L}(\pi^*|\boldsymbol{D}) + (\boldsymbol{\pi}-\boldsymbol{\pi}^*)^T \nabla \textup{L}(\boldsymbol{\pi}|\boldsymbol{D}) + \frac{1}{2}(\boldsymbol{\pi}-\boldsymbol{\pi}^*)^T H (\boldsymbol{\pi}-\boldsymbol{\pi}^*)^T.
\end{align*}
\end{enumerate}
\cite{Yang} shows that the QM condition holds true for least squares loss functions. The GMD algorithm uses the advantage of QM condition \ref{it:2}, where $\textup{L}(\boldsymbol{\pi}|\boldsymbol{D})$ can be further bounded using the largest eigenvalue of $H$. From the boundedness of $\textup{L}(\boldsymbol{\pi}|\boldsymbol{D})$ closed-form expression of $\hat{\boldsymbol{\pi}}$ can be derived for each of the $k$ groups $\boldsymbol{\pi}_k$, $k=1,\dots,G$. The algorithm uses block coordinate descent to cyclically update each group $\boldsymbol{\pi}_k$ until convergence.  

\section{Determination of regularization parameter $\lambda$} \label{sec:cvlambda}
In order to understand the relationship between the group lasso penalty $\lambda$ and $\balpha$, consider the decomposition of the $mean$ $square$ $error$ (MSE) of an estimator $\hat{\balpha}$ for $\balpha$. The MSE of $\hat{\balpha}$ is given by:
\begin{align*}
MSE(\hat{\balpha})=\textup{E}\left[(\hat{\balpha}-\balpha^*)^2 \right] = Bias(\hat{\balpha})^2 + \textup{Var}(\hat{\balpha}),
\end{align*}
where $\balpha^*$ is the true value of $\balpha$. This equality reveals a trade-off between the bias and variance. Larger values of $\lambda$ will force groups $\balpha_k$ with small values to be exactly $\boldsymbol{0}$ and thereby introduce a small variance for some groups. Even for groups that consists of zeros the bias will be zero for larger values of $\lambda$. However, at the same time the penalty will also introduce bias for groups $\balpha_k$ with non-zero values. Thus, the choice of $\lambda$ is rather difficult, due to this bias-variance trade-off.

In order to determine the value of $\lambda$ that minimizes the total estimation error among a sequence of pre-determined $\lambda$ values, we use a $K$-fold cross-validation procedure. We divide each $X_i$ into $K$ subsets of equal cardinality, i.e. $X_i=(X_{i,1}, \dots, X_{i,K})^T$ where $X_{i,j} \cap X_{i,k} = \emptyset$ for $j \neq k$. For each $c=1,\dots, K$ we define a $test$ $set$ $X_c=(X_{1,c}, \dots, X_{p,c})^T$ and a $training$ $set$ $X_{-c}=(X_{1,-c}, \dots, X_{p,-c})^T$ where $X_{i,-c}=X_i \backslash X_{i,c}$. From $X_{-c}$ we estimate $\btheta$ using \eqref{eq:penalize} for pre-determined values of $\lambda$. We denote by $\hat{\btheta}^{-c}(\lambda)$ the estimated $\btheta$ from $X_{-c}$. We now define a $K$-fold cross-validation procedure by:
\begin{align}
KCV(\lambda)=\frac{1}{K} \sum_{c=1}^K l_c(\hat{\btheta}^{-c}(\lambda)),
\end{align}
where 
\begin{align}
l_c(\hat{\btheta}^{-c}(\lambda)) = \sum_{i,j=1}^p\sum_{\substack{\bu \in X_{i,c} \\ \bv \in X_{j,c}}}^{\neq} \textup{log} \left( \textup{p}_{ij}\left( \bu,\bv;\hat{\btheta}^{-c}(\lambda)\right) \right) .
\end{align}
Thus, our estimate of $\lambda$ is given by:
\begin{align*}
\hat{\lambda}=\textup{arg max}_{\lambda} KCV(\lambda).
\end{align*}
The choice of $K$ must be taken carefully since a too large $K$ will make the cross-validation procedure very time consuming. Conversely, a too small $K$ will lead to inaccurate estimates of $\btheta^{-c}(\lambda)$.
%\section{Regularized estimation for semi-parametric model}
%However in order to impose groupwise sparsity within $\bold{\balpha}$ we add a penalizing term. Thus, we formulate the optimization problem as a concave regularization problem:
%\begin{align} \label{eq:object}
%Q(\btheta|\bbeta)=l(\btheta | \bbeta)-h_{\lambda}(\bold{\balpha}),
%\end{align}
%where $h_{\lambda}(\cdot)$ is a convex penalty function that depends on a non-negative tuning parameter $\lambda$. \textcolor{red}{specify the penalty function as a group LASSO that groupwise penalize $\balpha_{i\cdot}$ such that we can determine the correlation structure between the street crimes}. 
%
%\subsection{Asymptotic results}
%\textcolor{red}{Theoretical results to show :\\
%1) Consistent model selection? \\
%2) Is the estimator asymptotic normal distributed?\\
%3) Does the sparse $\balpha_i$ converge in probability to 0?}







==> sections/estimation1.tex <==
\section{Second order multinomial logistic regression} \label{sec:esti}
To obtain an estimate of the parameter vector $\btheta= \cup_{i=1}^p \btheta_i \in \R^{d}$, we consider a  second order conditional composite likelihood (CCL) approach. Since the estimation procedure in \cite{hessellund} provides consistent estimates of $\bbeta_i$, for $i=1,\dots,p-1$, we only focus on the parameter vector $\btheta$. Thus, we suppress the function arguments $\hat{\bbeta}$ in the rest of this paper and denote by $\hat{f}_i(\bu)=\textup{exp}(\hat{\bbeta}_i^T \bz(\bu))$. The idea is to generate probabilities for a random distinct pair of points, say $(\bu,\bv)$, to be from point process $X_i$ and $X_j$. We do that by defining the following second order conditional probabilities: 
\begin{align} \label{eq:proba}
\textup{p}_{ij}(\bu,\bv; \btheta) = \frac{\rho_{ij}(\bu,\bv;\btheta_{ij})}{\sum_{k , l= 1}^p \rho_{kl}(\bu,\bv;\btheta_{kl})} = \frac{\hat{f}_i(\bu) \hat{f}_j(\bv) g_{ij}(r; \btheta_{ij})}{\sum_{k , l= 1}^p \hat{f}_k(\bu) \hat{f}_l(\bv) g_{kl}(r; \btheta_{kl})},
\end{align} 
where $\rho_0(\bu)\rho_0(\bv)$ cancels out in \eqref{eq:proba}, hence the probabilities do not depend on $\rho_0(\cdot)$. Furthermore, we define a second order multinomial logistic likelihood (MLL) function by:
\begin{align} \label{eq:lik}
L(\btheta)= \prod_{i , j= 1}^p \prod_{\substack{\bu \in X_i \cap W \\ \bv \in X_j \cap W \\ ||\bu-\bv|| \leq R}}^{\neq} \textup{p}_{ij}(\bu,\bv; \btheta),
\end{align}
where $R \geq 0$. Notice that the constraint $||\bu-\bv|| \leq R$ reduces the computation time, but $R$ should still be chosen such that $g_{ij}(r) \approx 1$ for all $\bu,\bv$ with $||\bu-\bv||>R$.  The second order log-MLL function $l(\btheta)=\textup{log}(L(\btheta))$ is then:
\begin{align} \label{eq:loglik}
l(\btheta)=\sum_{i , j= 1}^p \sum_{\substack{\bu \in X_i \cap W \\ \bv \in X_j \cap W \\ ||\bu- \bv|| \leq R}}^{\neq} \textup{log}\left(\rho_{ij}(\bu,\bv;\btheta_{ij}) \right) -  \textup{log}\left( \sum_{k , l=1}^p \rho_{kl}(\bu,\bv;\btheta_{kl}) \right),
\end{align}
which is the object function with repect to
$\btheta$. Instead we turn \eqref{eq:loglik} into a minimization
problem and consider the negated second order log-MLL, denote by
$l_-(\btheta) = - l(\btheta)$, which we minimize with respect to
$\btheta$. The second order log-MLL function \eqref{eq:lik} has some resembles to a multinomial logistic regression likelihood function (of first order). However, in contrast to first order multinomial logistic regression problems we are not interested in reparameterization of each $\btheta_{ij}$ by choosing one parameter vector, say $\btheta_{mn}$, as a baseline in order to make each $\btheta_{ij}$ identifiable. The identifiability issue is simply accommodated due to the construction of the likelihood with $p^2$ probabilities $\textup{p}_{ij}(\bu,\bv;\btheta)$ for $\btheta$, which contains $p$ independent parameter vectors $\btheta_i$. Hence, the likelihood contains certain degrees of freedom to identify the parameters, but is still suffers from some identifiability issues as described in Section \ref{sec:ident}.


\subsection{Identifiability issues} \label{sec:ident}

Choose an arbitrary baseline pair of point processes, e.g.\
$(1,1)$. The probabilities \eqref{eq:proba} can then be rewritten as

\begin{align} \label{eq:proba2}
\textup{p}_{ij}(\bu,\bv; \btheta) =  \frac{\hat{f}_i(\bu) \hat{f}_j(\bv) g_{ij}(\bu,\bv; \btheta_{ij})/g_{11}(\bu,\bv; \btheta_{11})}{\sum_{k , l= 1}^p \hat{f}_k(\bu) \hat{f}_l(\bv) g_{kl}(\bu,\bv; \btheta_{kl})/g_{11}(\bu,\bv; \btheta_{ij})}.
\end{align}
Since 
\begin{align} \label{eq:crosspcf2}
\frac{g_{ij}(r;\btheta_{ij})}{g_{11}(r;\btheta_{11})}=\textup{exp}\left(
  \sum_{k=1}^q [\alpha_{ik} \alpha_{jk}- \alpha_{1k}^2]
  \textup{exp}\left(\frac{-r}{\xi_k} \right)+ 1[i=j]\sigma_i^2
  \textup{exp}\left(\frac{-r}{\phi_i} \right) - \sigma_1^2
  \textup{exp}\left(\frac{-r}{\phi_1} \right)\right)
\end{align}
our conditional likelihood function will provide information on the
$\alpha_{ij}$'s via the
differences $d_{ijk}=\alpha_{ik} \alpha_{jk}- \alpha_{1k}^2$. We can
then immediately observe an identifiability problem since if
$\alpha_{1k}=\ldots=\alpha_{qk}$ then all the $d_{ijk}$'s are
zero. Thus we can not reconstruct the $\alpha_{ik}$'s uniquely from
the $d_{ijk}$'s when the $d_{ijk}$'s are all zero. On the other hand,
if the $d_{ijk}$'s are consistent with at least one set of parameters
$\alpha_{ik}$, $i=1,\ldots,q$ where at least two parameters, say
$\alpha_l$ and $\alpha_{l'}$ differ,
then we can uniquely determine the $\alpha_{ik}$'s in question. This
follows easily by induction in $q$.

In conclusion, we have a lack of identifiability in the case where for
a $k$, the $\alpha_{ik}$ are all equal. Intuitively this makes sense,
because in this case the contribution from the field $Y_k$ is exactly
the same for all point processes whereby it can be absorbed into the
baseline function $\rho_0$. We can conceptually in this case regard
$Y_k$ as known and fixed since it cancels anyways when forming the
conditional probabilities. 

\subsection{Induction proof}
If $p=2$ then it is easy to see that $d_{12k}=\alpha_1
\alpha_2-\alpha_1^2$ and $d_{22k}=\alpha_{2}^2-\alpha_1^2$ has a
unique solution when $\alpha_{1k}\neq \alpha_{2k}$ (which implies that
we can assume $\alpha_{1k} \neq 0$). Assuming the result is ok for
$p=m$ we consider the case $p=m+1$. Without loss of generality we can
assume $\alpha_{1k} \neq \alpha_{2k}$ and $\alpha_{1k} \neq 0$. Thus
by induction we can recover $\alpha_{1k},\ldots,\alpha_{mk}$ from the
equations $d_{ijk}=\alpha_{ik}\alpha_{jk}-\alpha_{1}^2$ for $(i,j)\neq
(1,1)$ and $i<=j \leq k$. Finally we recover $\alpha_{k+1}$ from the
equation $d_{1(k+1)}=\alpha_1 \alpha_{k+1} - \alpha_1^2$.

\subsection{Cyclic coordinate descent algorithm} \label{sec:ccda}
%For the rest of this paper we consider $\btheta$ in terms of regularized and non-regularized parameters. We aim to regularize the cross-dependence parameters $\balpha$, while $\bpsi=(\xi,\bsigma^2,\bphi)^T$ is the parameter vector with no regularization. Thus, the estimation of $\balpha$ is treated seperately from $\bpsi$. 

In order to minimize $l_-(\btheta)$ with respect to $\btheta$, we consider a cyclic coordinate descent algorithm. The strategy is simply to update $\balpha$, $\xi$, $\bsigma^2$ and $\bphi$ in turn using \eqref{eq:loglik} until a convergence criterion is met. Denote by $\btheta^{(n)}=(\balpha^{(n)},\xi^{(n)},\bsigma^{2(n)},\bphi^{(n)})^T$ the current value of $\btheta$. Since we want to evaluate the correlation structure for a multivariate LGCP and determine sparse components, we regularize $\balpha$ using $lasso$ regression. Hence, for given values of $\xi^{(n)}$, $\bsigma^{2(n)}$  and $\bphi^{(n)}$ we update $\balpha$ by considering the following regularized log-MLL:  
\begin{align} \label{eq:penalize}
Q_{\lambda}(\balpha,\xi^{(n)},\bsigma^{2(n)},\bphi^{(n)}) = l_-(\balpha,\xi^{(n)},\bsigma^{2(n)},\bphi^{(n)}) + \lambda \sum_{i=1}^p \sum_{k=1}^q | \alpha_{ik} |,
\end{align} 
where $\lambda \sum_{i=1}^p \sum_{k=1}^q | \alpha_{ik} |$ is a lasso that serves to regularize each component in $\balpha$ for a given choice of the tuning parameter $\lambda$. In Section \ref{sec:cvlambda} we propose a cross-validation procedure to choose $\lambda$. In comparison to $ridge$ $regression$ with a L2-norm penalty, the lasso penalty is a L1-norm that can lead to zero coefficents. This makes lasso penalty not only helpful for over-fitting problems but also beneficial for model selection in comparison to ridge regression. %By using line search we update $\balpha^{(n+1)}=\balpha^{(n)} + t(\hat{\balpha}-\balpha^{(n)})$ such that $l_-(\balpha^{(n+1)},\bpsi^{(n)}) \leq l_-(\balpha^{(n)},\bpsi^{(n)})$ for some $t>0$. 
We update $\balpha^{(n+1)} = \balpha^{(n)} + t(\tilde{\balpha}-\balpha^{(n)})$ using a line search for some $t>0$, where $\tilde{\balpha}$ is obtained as the solution to 
\begin{align} \label{eq:argminalpha}
&\tilde{\balpha}= \textup{arg min}_{\balpha}  Q_{\lambda}(\balpha,\xi^{(n)},\bsigma^{2(n)},\bphi^{(n)}).
\end{align}
For the non-regularized parameter vectors we also update each parameter vector using line search, where $\tilde{\xi}$, $\tilde{\bsigma}^2$ and $\tilde{\bphi}$ are obtained as solutions to:
\begin{align} 
\tilde{\xi}&= \textup{arg min}_{\xi} l_-(\balpha^{(n+1)}, \xi,\bsigma^{2(n)},\bphi^{(n)}), \label{eq:argminxi}\\
\tilde{\bsigma}^2&= \textup{arg min}_{\bsigma^2} l_-(\balpha^{(n+1)}, \xi^{(n+1)},\bsigma^{2},\bphi^{(n)}) \textup{ and} \\
\tilde{\bphi}&= \textup{arg min}_{\bphi} l_-(\balpha^{(n+1)}\xi^{(n+1)},\bsigma^{2(n+1)},\bphi). \label{eq:argminphi}
\end{align}
The estimation procedures for \eqref{eq:argminalpha}-\eqref{eq:argminphi} are described in details in Section \ref{sec:algo}. Finally, $\hat{\btheta}:=\btheta^{(n+1)}$ is obtained as an estimate, when the algorithm convergence criterion is met. The coordinate descent algorithm is set to converge, whenever
\begin{align*}
\left\vert \frac{l_-(\btheta^{(n+1)})-l_-(\btheta^{(n)})}{l_-(\btheta^{(n)})} \right\vert < \epsilon,
\end{align*}
for some $\epsilon > 0$.

\subsection{Parameter updates using proximal Newton methods} \label{sec:algo}
In connection to first order multinomial logistic regression problems no closed form solutions exist for $\btheta$ using \eqref{eq:loglik}, hence we need to estimate the parameters using iterative procedures. Following \cite{lee} we can minimize \eqref{eq:argminalpha}-\eqref{eq:argminphi} using proximal Newton methods. The concept is basically to approximate the likelihood using a second order Taylor expansion and replace the hessian matrix by a positive definite matrix. By minimizing the second order approximation of the likelihood with additional line search, Proposition 2.3 in \cite{lee} ensures that the parameter updates will always decrease the value of the likelihood function. For a general exposure of the concept, we consider some $\bpsi \in \{\balpha, \xi,\bsigma^2,\bphi \}$ as the parameter vector of interest and $\bpi = \btheta \backslash \bpsi$ as the remaining (fixed) parameters. Now, consider a second order Taylor approximation of $l_-(\bpsi,\bpi^{(n)})$ with respect to $\bpsi$ and with initial parameters $\bpsi^{(n)}$ and $\bpi^{(n)}$:
\begin{align} \label{eq:taylor}
f(\bpsi,\bpi^{(n)}) & = l_-(\btheta^{(n)}) + (\bpsi - \bpsi^{(n)})^T\best(\btheta^{(n)}) + \frac{1}{2}(\bpsi - \bpsi^{(n)})^T \textup{H} (\btheta^{(n)})(\bpsi - \bpsi^{(n)}).
\end{align} 
We now aim to update $\bpsi$ using the second order Taylor expansion, since $\tilde{\bpsi} \approx \textup{arg min}_{\bpsi} \left(f(\bpsi,\bpi^{(n)}) \right)$ is an approximate solution to \eqref{eq:argminxi}-\eqref{eq:argminphi}. The function
\begin{align} \label{eq:estfct}
\best(\btheta^{(n)})  =\nabla_{\bpsi}l_-(\btheta^{(n)})= \sum_{i , j=1}^p \sum_{\substack{\bu \in X_i \cap W \\ \bv \in X_j \cap W \\ ||\bu -\bv|| \leq R}}^{\neq} \left( \frac{\sum_{k , l= 1}^p \nabla_{\bpsi} \rho_{kl}(\bu,\bv;\btheta^{(n)})}{\sum_{k , l =1}^p  \rho_{kl}(\bu,\bv;\btheta^{(n)})} - \frac{\nabla_{\bpsi} \rho_{ij}(\bu,\bv;\btheta^{(n)})}{\rho_{ij}(\bu,\bv;\btheta^{(n)})} \right)
\end{align}
is the estimating function with respect to $\bpsi$. Notice that \eqref{eq:estfct} does not depend on $\rho_0(\bu)\rho_0(\bv)$. Moreover, Lemma \ref{lem:unb} show that $\best(\btheta^*)$ is an unbiased estimating function. The function 
\begin{align} \label{eq:ehess}
\textup{H}(\btheta^{(n)})=\textup{E} [\nabla^2_{\bpsi} l_-(\btheta^{(n)})] = \int_{W^2} 1_R \textup{Cov} \left(X(\bu,\bv;\btheta^{(n)}) \right) \sum_{i , j= 1}^p \rho_{ij}(\bu,\bv;\btheta_{ij}^{(n)}) \textup{d} \bu \textup{d} \bv
\end{align}
is the expected hessian with respect to $\bpsi$, where $1_R=1[||\bu-\bv || \leq R]$ and $X(\bu,\bv;\btheta^{(n)}) $ denote a random vector which takes values $\nabla_{\bpsi} \textup{log}(\rho_{ij}(\bu,\bv;\btheta^{(n)}))$ with probability $\textup{p}_{ij}(\bu,\bv;\btheta^{(n)})$. The expression of \eqref{eq:ehess} is derived in Lemma \ref{prop:sens}. We approximate \eqref{eq:ehess} using \eqref{eq:campbell}:
\begin{align*}
\hat{H}(\btheta^{(n)})=\sum_{i , j= 1}^p \sum_{\substack{\bu \in X_i \cap W \\ \bv \in X_j \cap W \\ ||\bu -\bv|| \leq R}}^{\neq} \textup{Cov} \left(X(\bu,\bv;\btheta^{(n)}) \right),
\end{align*}
which is an unbiased estimate of $\textup{H}(\btheta^{(n)})$ that does not depend on $\rho_0(\bu)\rho_0(\bv)$. Since $\textup{H}(\btheta^{(n)})$ is a symmetric, positive semi-definite matrix, the eigendecomposition implies that $\textup{H}(\btheta^{(n)})^{1/2}=UD^{1/2}U^T$, where $D^{1/2}=\textup{diag}(\textup{l}^{1/2})$ with $\textup{min}(\textup{l}) \geq 0$ and the columns of $U$ correspond to the eigenvectors of $\textup{H}(\btheta^{(n)})$. Due to Appendix \ref{app:pnm} we can rethink \eqref{eq:argminxi} - \eqref{eq:argminphi} as approximate solutions to least squares problem:
\begin{align} \label{eq:minfct2}
\tilde{\bpsi} \approx \textup{arg min}_{\bpsi} \bigg( \frac{1}{2} ||Y -X\bpsi ||^2 \bigg) ,
\end{align}
where
\begin{align*}
Y&=\hat{\textup{H}}(\btheta^{(n)})^{1/2}\left( -\hat{\textup{H}}(\btheta^{(n)})^{-1}\best(\btheta^{(n)})+\btheta^{(n)} \right) \quad \textup{and} \\
X&=\hat{\textup{H}}(\btheta^{(n)})^{1/2}.
\end{align*}
In the case $\bpsi:=\xi,\bsigma^2,\bphi$ or $\bpsi:=\balpha$ for $\lambda=0$ the OLS (ordinary least squares) estimator minimizes \eqref{eq:minfct2}, i.e. we update $\tilde{\bpsi}$ by
\begin{align}
\tilde{\bpsi} \leftarrow (X^TX)^{-1} X^TY,
\end{align}
given that the columns of $X$ are linearly independent.
In the case $\bpsi:=\balpha$ for $\lambda > 0$, our approximate solution to \eqref{eq:argminalpha} is then given by:
\begin{align*}
\tilde{\balpha} \approx \textup{arg min}_{\balpha} \bigg( \frac{1}{2} ||Y -X\balpha ||^2  + \lambda \sum_{i=1}^p \sum_{k=1}^q | \alpha_{ik} | \bigg).
\end{align*}
Following \cite{fried2} we update $\alpha_i$ by
\begin{align}
\alpha_i \leftarrow \frac{S \left( X_{\cdot i}^T \left(Y - \sum_{j \neq i} X_{\cdot j} \alpha_j^{(n)} \right), \lambda \right)}{ X_{\cdot i}^T X_{\cdot i}},
\end{align}
where $X_{.j}$ is the j'th column of $X$ and $S(c,\lambda)$ is a soft-thresholding operator given by:
\begin{align*}
S(c,\lambda)= \begin{cases} c - \lambda &\textup{ if } c>0 \textup{ and } \lambda < |c| \\
 c+\lambda &\textup{ if } c<0 \textup{ and } \lambda < |c| \\
 0 &\textup{ if } \lambda > |c|.
\end{cases}
\end{align*}


\section{Determination of $q$ and $\lambda$} \label{sec:cvlambda}
In order to understand the relationship between the lasso penalty $\lambda$ and $\balpha$, consider the decomposition of the $mean$ $square$ $error$ (MSE) of an estimator $\hat{\balpha}$ for $\balpha$. The MSE of $\hat{\balpha}$ is given by:
\begin{align*}
MSE(\hat{\balpha})=\textup{E}\left[(\hat{\balpha}-\balpha^*)^2 \right] = Bias(\hat{\balpha})^2 + \textup{Var}(\hat{\balpha}),
\end{align*}
where $\balpha^*$ is the true value of $\balpha$. This equality reveals a trade-off between the bias and variance. Larger values of $\lambda$ will force some $\hat{\alpha}_{ik}$ with small value to be exactly $0$ and thereby introduce a small variance. However, at the same time the penalty will also introduce bias for other $\hat{\alpha}_{jk}$ with non-zero value. Thus, the choice of $\lambda$ is rather difficult, due to this bias-variance trade-off.

In order to determine the value of $q$ and $\lambda$ that minimizes the total estimation error among sequences of pre-determined values of $q$ and $\lambda$, we use a $K$-fold cross-validation procedure with $N$ resamplings. Given a realization $X=\boldsymbol{x}$ with $n$ points $\boldsymbol{x}=(\boldsymbol{x}_1, \dots, \boldsymbol{x}_n)$ we sample $c_i=n(K-1)/K$ points independently from $\boldsymbol{x}$, say $\boldsymbol{x}_{c_i}$, and denote by $\boldsymbol{x}_{-c_i} = \boldsymbol{x} \backslash \boldsymbol{x}_{c_i}$ the point realization with $-c_i=n/K$ points. The indices $i$ indicate the i'th resampling of $\boldsymbol{x}$. From $\boldsymbol{x}_{c_i}$ we estimate $\btheta$ using the algorithm described in \ref{sec:ccda} for values of $q$ and $\lambda$. We denote by $\hat{\btheta}^{c_i}(q,\lambda)$ to stress that $\btheta$ is estimated using $\boldsymbol{x}_{c_i}$, $q$ and $\lambda$. The cross-validation score  for $\hat{\btheta}^{c_i}(q,\lambda)$ is then:
\begin{align*}
CV(\hat{\btheta}^{c_i}(q,\lambda))= -\sum_{k,l=1}^p\sum_{\substack{\bu \in \boldsymbol{x}_{k,-c_i} \\ \bv \in \boldsymbol{x}_{l,-c_i} \\ ||\bu -\bv|| \leq R}}^{\neq} \textup{log} \left( \textup{p}_{kl}\left( \bu,\bv;\hat{\btheta}^{c_i}(q,\lambda)\right) \right),
\end{align*}
for some $R$. By doing N independent samplings of $\boldsymbol{x}_{c_i}$ we now define a $K$-fold cross-validation procedure with $N$ resamplings by:
\begin{align}
KNCV(q,\lambda)=\frac{1}{N} \sum_{i=1}^N CV(\hat{\btheta}^{c_i}(q,\lambda)),
\end{align}

Thus, our estimate of $q$ and $\lambda$ are given by:
\begin{align*}
(\hat{q},\hat{\lambda})=\textup{arg min}_{q,\lambda} KNCV(q,\lambda).
\end{align*}
The choice of $K$ and $N$ must be taken carefully since a too large values of $K$ and $N$ will make the cross-validation procedure very time consuming. Conversely, a too small $K$ will lead to inaccurate estimates of $\btheta^{-c_i}(q,\lambda)$.
%\section{Regularized estimation for semi-parametric model}
%However in order to impose groupwise sparsity within $\bold{\balpha}$ we add a penalizing term. Thus, we formulate the optimization problem as a concave regularization problem:
%\begin{align} \label{eq:object}
%Q(\btheta|\bbeta)=l(\btheta | \bbeta)-h_{\lambda}(\bold{\balpha}),
%\end{align}
%where $h_{\lambda}(\cdot)$ is a convex penalty function that depends on a non-negative tuning parameter $\lambda$. \textcolor{red}{specify the penalty function as a group LASSO that groupwise penalize $\balpha_{i\cdot}$ such that we can determine the correlation structure between the street crimes}. 
%
%\subsection{Asymptotic results}
%\textcolor{red}{Theoretical results to show :\\
%1) Consistent model selection? \\
%2) Is the estimator asymptotic normal distributed?\\
%3) Does the sparse $\balpha_i$ converge in probability to 0?}







==> sections/introduction.tex <==
\section{Introduction}
In the last decades large amounts of collected data and the improved computational speed have founded various statistical methods for selection of regression models. Such selection methods includes Akaike information criterion (AIC) and Bayesian information criterion (BIC) that estimates the quality of statistical models for given data and thereby can be used for comparison of models. 

Other kinds of selection methods involves regularization techniques, that in general can be characterized as an optimization problem of a regression model with an additional penalty function. The specification of such penalty function lead to different classes of regularization methods. \cite{tibshirani} introduced the popular $least$ $absolute$ $shrinkage$ $and$ $selection$ $operator$ (lasso) for linear models as a method to minimize the residual sum of squares. With the constraint of the lasso some of the parameter estimates can be forced to be exactly $0$, which makes the regression model very interpretable for selection of parameters. Moreover, this feature of forcing parameters to be exactly 0 makes the lasso method very appealing compared to other regularization methods like $ridge$ regression. \cite{Yuan} extented the lasso to a group variable version, called $group$ $lasso$, and provided an estimation algorithm based on $least$ $angle$ $regression$ $selection$ (LARS). This was further extended by \cite{fried2} that proposed a group lasso term and a sparse group lasso for linear models. \cite{fried2} developed an estimation algorithm based on cyclic co-ordinate descent updates. \cite{meier} considered the group lasso in relation to logistic regression, where they proposed an optimization algorithm using block co-ordinate descent updates to solve convex problems. In their approach they penalized an approximation of the log-likelihood function using a second order Taylor expansion and then considered the minimization with respect to groups of parameters. \cite{fried1} proposed a fast $elastic$ $net$ algorithm for generalized linear models. This algorithm includes cyclic coordinate descent updates and derived criterions for updating the parameter of interest.

Also regularization methods in relation to the spatial point processes framework have been developed. \cite{choiruddin1} considered regularization problems for the intensity functions of spatial point processes. In particular, they considered Poisson likelihood and logistic regression likelihood and assumed that the intensity is parameterized and has a log-linear specification. Moreover, \cite{choiruddin2} considered regularization problems for highly multivariate log Gaussian Cox processes (LGCP).

In this paper we want to infer the second order structures for a multivariate spatial point processes that is observed in an heterogeneous environment. The motivating example is street crime data that is considered as point pattern data generated from inhomogeneous point processes. For both crimonologists, police service or public perspectives the information of how street crimes are spatially dependent on each other is of great interest, since this knowlegde can lead to initiatives against street crime occurrences. The intensity function of each street crime is complex to model, since it depends on the layout of the city as well as the typically unknown population density at any location. To accommodate this issue we assume a semi-parametric regression model, where the intensity function of a street crime is represented as a function of a non-parametric term common to all the street crimes and a parametric term which models the influence of demographical covariates on the street crimes. Methods to infer first order structures of street crimes are already studied in \cite{hessellund}. By inferring the second order parameters of the street crimes we are able to investigate the spatial dependence between each crime types. We assume that the street crimes can be modeled by a multivariate LGCP as considered in \cite{Waage}. These types of Cox processes has simple expressions for the cross-pair correlation function (cross-PCF) and are flexible with regard to modelling point patterns with cross dependence. However, computational problems might occur if we want to obtain confidence intervals derived from the asymptotic normal distribution and the covariance matrix of the second order parameters. The estimation of the covariance matrix depends on fourth order sums, which makes the estimation procedure very time consuming and numerically unstabile. 

Instead we consider a second order conditional composite likelihood function with a penalizing term, that serves to regularize the cross-dependence parameters. Our approach is inspired by \cite{meier} and \cite{lee}, where we use proximal Newton methods to minimize our negated second order conditional composite likelihood with an added penalizing term. For computation we use the R package \texttt{gglasso} proposed by \cite{Yang}. This R package contains a fast unified algorithm for group lasso penalize problems. With our approach we aim to regularize the cross-dependence parameters and thereby determine the spatial correlations between each pair of street crimes.

The rest of the paper is organized as follows. Section \ref{sec:back} gives a brief overview of multivariate point processes with focus on the intensity functions and cross intensity functions. This is followed by a brief introduction to the semi-parametric model for the intensity function in Section \ref{sec:semi} and a overview of multivariate LGCP's in Section \ref{sec:mlgcp}. In Section \ref{sec:esti} we propose our second order conditional composite likelihood function with focus on how to estimate the cross-dependence parameters using proximal Newton methods for the negated likelihood in Section \ref{sec:algo}. This is followed by a detailed description of the $groupwise$ $majorization$ $descent$ (GDM) algorithm proposed by \cite{Yang} In Section \ref{sec:gdm}. In Section \ref{sec:cvlambda} we provide a cross-validation method to determine the value of the penalty parameter while Section \ref{sec:simu} contains simulation studies of our estimation approach. Section \ref{sec:dataanalysis} contains a study of Wastington DC. as a data example of our estimation approach, while Section \ref{sec:con} gives some concluding remarks.  

\section{Background} \label{sec:back}
\noindent Let $X=(X_1, \dots, X_p)$ be a multivariate spatial point process, where each $X_i$ is a spatial point process on $\R^d$ and each point $\bu \in X_i$ corresponds to an event $\bu \in \R^d$. In practice, we observe each $X_i$ in a spatial window $W$, where the window $W \subset \R^d$ is bounded with area $|W|>0$. Assume that there for each $i,j=1,\dots,p$ exists a non-negative functions $\rho_{i}(\cdot)$ and $\rho_{ij}(\cdot)$ so that:
\begin{align}\label{eq:crossprod}
\textup{E} \sum_{\bu \in X_i}  1[\bu \in A] &= \int_{A} \rho_{i}\left( \bu\right) \textup{d}\bu \\
\textup{E} \sum_{\bu \in X_i,\bv \in X_j}^{\neq}  1[\bu \in A, \bv \in B] &= \int_{A \times B} \rho_{ij}\left( \bu,\bv \right) \textup{d}\bu \textup{d}\bv,
\end{align}
\noindent where $A,B \subset \R^d$ and $\sum^{\neq}$ means that $\bu,\bv$ are pairwise distinct. The function $\rho_{i}(\cdot)$ is called the intensity function of $X_i$. If $i=j$, then $\rho_{ii}(\cdot)$ is called the second order intensity function of $X_i$. Moreover, if $i \neq j$ then $\rho_{ij}(\cdot)$ is called the cross intensity function between $X_i$ and $X_j$. For two infinitesimally small balls with centers $\bu,\bv$ and volumes $\textup{d}\bu,\textup{d}\bv$, $\rho_{ij}\left( \bu,\bv \right) \textup{d}\bu \textup{d}\bv$ is the joint probability of observing an event in each of the two small balls. The normalized cross intensity function, called cross pair correlation function (cross PCF), is denoted by $g_{ij}(\cdot)$ and defined by: 
\begin{align} \label{eq:pcf}
\rho_i(\bu) \rho_j(\bv) g_{ij}(\bu,\bv)=\rho_{ij}\left(\bu,\bv \right),
\end{align}
if both $\rho_i(\bu)$, $\rho_j(\bv)$ and $\rho_{ij}(\bu,\bv)$ exists. If $i=j$ we just call $g_{ii}(\cdot)$ the pair correlation function (PCF). If $X_i$ and $X_j$ are independent, then $g_{ij}=1$. Hence the cross PCF provides useful insight of the cross dependence between two point processes. Furthermore, to analyze the spatial dependence within a point process $X_i$, one can compare distribution of $X_i$ with the  distribution of the Poisson point process. Poisson point processes play an essential role in spatial statistics as a class of model for generating point patterns with complete spatial randomness. A fundamental result for a Poisson point process shows that its PCF equals one. Thus, $g_{ii}(\cdot)>1$ ($g_{ii}(\cdot)<1$) means that $X_i$ is more (less) clustered than a Poisson process with the same intensity function. For the rest of this paper we assume that the multivariate point process is second order cross-intensity reweighted stationary, i.e. $g_{ij}(\bu,\bv)=g_{ij}(r)$, where $r=||\bu-\bv||$.

A useful result for this paper is the so-called $cross$ $Campbells$ $formula$, which states the following equality:
\begin{align} \label{eq:campbell}
\textup{E} \sum_{\bu \in X_i,\bv \in X_j}^{\neq}  h(\bu,\bv) &= \int_{A \times B} h(\bu,\bv) \rho_{ij}\left( \bu,\bv \right) \textup{d}\bu \textup{d}\bv,
\end{align}
where $h(\bu,\bv)$ is a non-negative function. Similar statement hold for $i=j$.

\subsection{Semi-parametric regression model for the intensity} \label{sec:semi}

For spatial point pattern data in heterogeneous environment with a complex observation window, the intensity function of each point process is rather complex to model. For instance, when considering  street crime data the street crimes can only occur in streets, parks, and other public spaces. Moreover, the intensity for street crimes at a given location depends on the population density - if nobody is around, crimes will not happen. We denote by $\rho_{0}(\cdot)$ a background intensity function that incorporates effects of the complex observation window and is assumed to be common for all point types. We then propose the multiplicative model
\begin{align} \label{eq:multi1}
\rho_{i}(\bu; \bgamma_i)=\rho_{0}(\bu) \exp(\bgamma_i^\T \bz(\bu) )
\end{align} 
for the intensity of $X_i$ where $\bz(\bu)$ denotes a $q$-dimensional
vector of spatial covariates at location $\bu$ and $\bgamma_i \in \R^q$ is a
regression parameter. \cite{hessellund} proposed an estimation procedure for model \eqref{eq:multi1}, where the relative effects of the covariates are estimated. More precisely, we choose a baseline point process, say $X_p$, and then estimate the differences $\bbeta_i=\bgamma_i-\bgamma_p$ for each $i = 1, \dots, p-1$ of the covariate vector $\bz(\bu)$. Thus, we estimate the relative risk $r_{ip}(\bu)=\rho_i(\bu)/\rho_p(\bu)$. The relative risk $r_{ip}(\bu)$ tells how more or less likely is it that a point process of type $i$ happens at $\bu$ relative to the baseline point process of type $p$. However, the main focus in this paper is not to infer $\bbeta_i$ but instead to infer the second order structures of the multivariate point process. We do so by assuming that the multivariate point process can be modeled as a multivariate LGCP, which is described in details in Section \ref{sec:mlgcp}.

\subsection{Multivariate log Gaussian Cox model}\label{sec:mlgcp}

Following the setup in \citet{Waage}, we assume that $X_i$ for $i=1,\dots, p$ has a random intensity given by:
\begin{align} \label{eq:lgcpint}
\Lambda_i(\bu)= \rho_0 (\bu) \exp(\bgamma_i^\T \bz(\bu))\textup{exp}\left(\mu_i + \sum_{k=1}^q\alpha_{ik} Y_k(\bu)+ \sigma_i U_i(\bu) \right),
\end{align} 
where $Y_k(\bu)$ and $U_i(\bu)$ are all independent zero-mean unit variance Gaussian random fields, $\rho_0(\bu)$ is the inhomogeneous background intensity and $\mu_i= \textup{log}(N_i)- \sum_{k=1}^q\alpha_{ik}^2/2 - \sigma_i^2/2$. The parameter $N_i$ determines the expected number of point within each point process. We can consider $Y_k(\cdot)$ as latent random fields that effects all types of points, hence the different types of points are correlated due to the dependence on $Y_k(\cdot)$. Moreover, we can consider $U_i(\cdot)$ as a type-specific random field that only effects the $i$'th type of points, hence $U_i(\cdot)$ models the clustering within each $X_i$. The expectation of \eqref{eq:lgcpint} is
\begin{align*}
\textup{E} [\Lambda(\bu)]& = \rho_0(\bu) \exp(\bgamma_i^\T \bz(\bu)) \textup{exp}(\mu_i) \textup{E} [ \textup{exp}(\sum_{k=1}^q \alpha_{ik} Y_k(\bu))] \textup{E} [ \textup{exp}(\sigma_i U_i(\bu))] \\
&= \rho_0(\bu) \exp(\bgamma_i^\T \bz(\bu)),
\end{align*} 
which follows from the moment generating function of a Gaussian random variable. Moreover, in a similar way it can be shown that:
\begin{align*}
\textup{E} [\Lambda_i(\bu)\Lambda_j(\bv)] = &  \rho_0(\bu)  \rho_0(\bv) \exp(\bgamma_i^\T \bz(\bu))\exp(\bgamma_j^\T \bz(\bu)) \\
& \times \textup{exp}\left(\sum_{k=1}^q \alpha_{ik} \alpha_{jk} c_{Y_k}(\bu,\bv) + 1[i=j] \sigma_i^2 c_{U_i}(\bu,\bv) \right),
\end{align*}
where $c_{Y_k}(\bu,\bv)=\textup{Corr}[Y(\bu),Y(\bv)]$ and $c_{U_i}(\bu,\bv)=\textup{Corr}[U_i(\bu),U_i(\bv)]$. For $c_{Y}(\cdot)$ and $c_{U_i}(\cdot)$ we use exponential correlation functions, i.e. $c_{Y_k}(\bu,\bv)=\textup{exp}(-||\bu-\bv||/\xi_k)$ and $c_{U_i}(\bu,\bv)=\textup{exp}(-||\bu-\bv||/\phi_i)$ with $\xi_k$ and $\phi_i$ as correlation scale parameters. Denote by $\btheta_i = (\balpha_i,\bxi, \sigma_i^2,\phi_i) \in \R^{2(q+1)}$, where $\balpha_i=(\alpha_{i1},\dots, \alpha_{iq})^T$ and $\bxi=(\xi_1, \dots, \xi_q)^T$. Thus, the cross-PCF between $X_i$ and $X_j$ is given by the parametric model:
\begin{align} \label{eq:crosspcf1}
g_{ij}(r;\btheta_{ij})=\textup{exp}\left(\sum_{k=1}^q \alpha_{ik} \alpha_{jk} \textup{exp}\left(\frac{-r}{\xi_k} \right)+ 1[i=j]\sigma_i^2 \textup{exp}\left(\frac{-r}{\phi_i} \right) \right),
\end{align}
where $\btheta_{ij}=\btheta_{i} \cup \btheta_{j}=(\balpha_i,\balpha_j, \bxi ,\sigma_i^2,\sigma_j^2,\phi_i,\phi_j)$. If $\sum_{k=1}^q\alpha_{ik} \alpha_{jk}$ is greater (smaller) than $0$, it implies positive (negative) spatial correlation between points from $X_i$ and $X_j$. If $\sum_{k=1}^q \alpha_{ik} \alpha_{jk}=0$ then $X_i$ and $X_j$ are independent. 

Regarding $\rho_0(\cdot)$ we obtain this as a realization of 
\begin{align*}
\Lambda_0(\bu)=\textup{exp} \left( \pi V(\bu) - \frac{\pi^2}{2} \right)
\end{align*}
where $V(\bu)$ a zero-mean unit variance Gaussian random field, independent of $Y_k$ and the $U_i$. By taking a closer look at \eqref{eq:crosspcf1}, we are not able to identify each $\alpha_{i}$  without imposing some constraints, since $\alpha_{ik}$ is composed in the product $\alpha_{ik} \alpha_{jk}$ in the cross-PCF. This only allow us to estimate $|\alpha_{i}|$. However, since we are only interested in evaluating the spatial correlation between each $X_i$ and $X_j$, we only need to estimate the product $\alpha_{ik} \alpha_{jk}$, which fortunately is tractable. Throughout this paper we denote by $\balpha$ a $p \times q$ matrix with entries $\alpha_{ik}$ for $i=1 \dots   p$ and $k =1 \dots q$. 




==> sections/penalized.tex <==
%\section{Regularized regression for semi-parametric model}
%In the following we consider a cross-conditional composite likelihood approach with a penalizing term. Define the probabilities: 
%\begin{align} \label{eq:proba}
%\textup{p}_{ij}(u,v; \theta | \beta) = \frac{\lambda_{ij}(u,v;\theta_{ij} | \beta_{ij})}{\sum_{k , l=1}^{p} \lambda_{kl}(u,v;\theta_{kl} | \beta_{kl})} = \frac{f(u;  \beta_i) f(v; \beta_j) g_{ij}(u,v; \theta_{ij})}{\sum_{k , l=1}^p f(u; \beta_k) f(v; \beta_l) g_{kl}(u,v; \theta_{kl})},
%\end{align} 
%where $\lambda_0(u)\lambda_0(v)$ cancels out in \eqref{eq:proba}, hence the probabilities do not depend on $\lambda_0(\cdot)$. Furthermore, we define a cross-conditional composite likelihood function by:
%\begin{align*}
%L(\theta | \beta)= \prod_{i , j=1}^p \prod_{\substack{u \in X_i \cap W \\ v \in X_j \cap W \\ ||u-v|| \leq R}}^{\neq} \textup{p}_{ij}(u,v; \theta | \beta),
%\end{align*}
%where $R \geq 0$. The cross-conditional composite log-likelihood function $l(\theta | \beta)=\textup{log}(L(\theta | \beta))$ is then:
%\begin{align*}
%l(\theta | \beta)=\sum_{i , j=1}^p \sum_{\substack{u \in X_i \cap W \\ v \in X_j \cap W \\ ||u- v|| \leq R}}^{\neq} \textup{log}\left(\lambda_{ij}(u,v;\theta_{ij} | \beta_{ij}) \right) -  \textup{log}\left( \sum_{k,l=1}^p \lambda_{kl}(u,v;\theta_{kl} | \beta_{kl}) \right)  .
%\end{align*}
%
%
%
%
%\section{LASSO for linear models}
%Let $(X_i,Y_i)$ be i.i.d random pairs following the linear regression model: 
%\begin{align*}
%Y_i = X_i \beta + \epsilon_i,
%\end{align*}
%where $X_i=(X_{i1},\dots,X_{ip})^T$ is a $p_n$-dimensional vector distributed as $N(0,\Sigma)$, $\beta=(\beta_1,\dots, \beta_p)^T$ is the true regression cofficients and $\epsilon_i \sim N(0,\sigma^2)$ is i.i.d. The LASSO is defined as:
%\begin{align*}
%\hat{\beta}= \textup{arg min}_{\beta} \left((2n)^{-1} \sum_{i=1}^n (Y_i - X_i^T \beta)^2 + \lambda_n \sum_{j=1}^{p_n} |\beta_n| \right),
%\end{align*}
%where $\lambda_n$ are tuning parameters. For consistency of the model selection and sensitivity of $\lambda_n$, Wainwright has identified precise conditions of achieving sparsity recovery with a family of regularization parameters $\lambda_n$ under deterministic setup.
%
%\section{LASSO for logistic models}

\section{Questions}
\begin{itemize}
\item How to choose $\lambda_k$ such that the penalized estimating function is consistent?

\item Can we show that estimating function is unbiased? Because the penalized version has discontinous points, an exact solution may not exist. Therefore we use Newton-type methods for minimizing the penalized estimating function.

\item How to show constency?

\item How to show asymptotic normality?

\item explain the basic idea of $\lambda_k$, i.e. how do they work in practice.

\end{itemize}



==> sections/simulation.tex <==
\section{Simulation study} \label{sec:simu}
We study the performance of the algorithm described in Section \ref{sec:ccda} on a multivariate LGCP on a fixed window $W$ with a sparse correlation structure. We study the algorithm over a sequence of common latent fields $q$ and lasso penalties $\lambda$, as the method for selecting the right number of latents fields and the sparse components within the correlation structure is non-trivial. As highlighted in Section \ref{sec:mlgcp} only products $\alpha_{ik}\alpha_{jk}$ is identifiable, hence we consider $\boldsymbol{A} =\balpha \balpha^T$ as the matrix with parameters of interest. The $i,j$'th entry of $\boldsymbol{A}$ reveals how $X_i$ and $X_j$ spatially correlates. We validate the performance of the algorithm using $root$ $mean$ $squared$ $error$ (RMSE) of each estimated parameter vector $\hat{\bpsi} \in \{\hat{\boldsymbol{A}},\hat{\bxi}, \hat{\bsigma}^2,\hat{\bphi}\}$, i.e:
\begin{align*}
RMSE(\hat{\bpsi})=\sqrt{\textup{E}\left[(\hat{\bpsi}-\bpsi^*)^2 \right]}.
\end{align*}
To determinate the number of common latent fields $q$ and the value of penalty parameter $\lambda$ we suggest the cross-validation procedure as described in Section \ref{sec:cvlambda}. The simulation settings are described in detailed in the following section.

\subsection{Five-variate LGCP with sparse correlation structure}
We simulate $100$ five-variate LGCP's $\bold{X}=(X_1,X_2,X_3,X_4,X_5)^T$ on $W=[0,1]^2$. Recall, the cross-PCF between $X_i$ and $X_j$ is a parametric function given by: 
\begin{align} 
g_{ij}(r;\btheta_{ij})=\textup{exp}\left(\sum_{k=1}^2 \alpha_{ik} \alpha_{jk} \textup{exp}\left(\frac{-r}{\xi_k} \right)+ 1[i=j]\sigma_i^2 \textup{exp}\left(\frac{-r}{\phi_i} \right) \right).
\end{align}
In this setup we have two common latent fields $Y_1$ and $Y_2$ along with one covariate $Z$ and background intensity $\lambda_0$. The realization of $Z$ and $\lambda_0$ can be found in Figure \ref{fig:latfields} along with plots of the PCF's and cross-PCF's.
\begin{figure}[ht!]
\centering
\begin{tabular}{c c c c}
\includegraphics[scale=0.20]{figures/simulation/2020-05-28/covariate.pdf}
\includegraphics[scale=0.20]{figures/simulation/2020-05-28/background_int.pdf}
\includegraphics[scale=0.20]{figures/simulation/2020-05-28/true_pcf.pdf}
\includegraphics[scale=0.20]{figures/simulation/2020-05-28/true_cross_pcf.pdf}
\end{tabular}
\caption{From left to right: Realization of $Z$ and $\lambda_0$, plots of PCF's and non-zero cross-PCF's.} \label{fig:latfields}
\end{figure}
The true parameter values of each $X_i$ can be found in Table \ref{tab:lgcp}. 
\begin{figure}[ht!]
\centering
\begin{tabular}{| c | c c |c  c  c  c  c  c  c |}
\hline
$X$ & $\bgamma_1^*$ & $\bgamma_2^*$ & $\balpha_{1}^*$ & $\balpha_{2}^*$ & $\xi_1^*$ & $\xi_2^*$ & $\bsigma^{2*}$ & $\bphi^*$ & $N_i$ \\
  \hline
  $X_1$ & 0.1 & -0.1 & 0 & 0 & 0.02 & 0.03 & $0.5$ & 0.02 & 400 \\
  $X_2$ & 0.2 & -0.2 & 1 & 0 & 0.02 & 0.03 & $0.5$ & 0.02 & 400 \\
  $X_3$ & 0.3 & 0 & 1 & 0 & 0.02 & 0.03 & $0.5$ & 0.03 & 400\\
  $X_4$ & 0.4 & 0.1 & 0 & -1 & 0.02 & 0.03 & $0.5$ & 0.03 & 400\\
  $X_5$ & 0.5 & 0.2 & 0 & 1 & 0.02 & 0.03 & $0.5$ & 0.04 & 400\\
  \hline
\end{tabular}
\caption{Simulation settings for $X$.} \label{tab:lgcp}
\end{figure}
Notice that $X_2$ and $X_3$ are positive spatial correlated, while $X_4$ and $X_5$ are negatively spatial correlated. In order to reduce the computation time, we only consider distinct pairs of points $\bu,\bv \in \bold{X}$ with $||\bu-\bv|| \leq 0.1$. All first order parameters are estimated using the estimation procedure in \cite{hessellund}, where we choose $X_1$ as the baseline point process. Histogram plots of $\hat{\bbeta}_1$ and $\hat{\bbeta}_2$ can be found in Figure \ref{fig:betahat}.
\begin{figure}[ht!]
\centering
\begin{tabular}{c c c c}
\includegraphics[scale=0.20]{figures/simulation/2020-05-28/beta11.pdf}
\includegraphics[scale=0.20]{figures/simulation/2020-05-28/beta21.pdf}
\includegraphics[scale=0.20]{figures/simulation/2020-05-28/beta31.pdf}
\includegraphics[scale=0.20]{figures/simulation/2020-05-28/beta41.pdf} \\
\includegraphics[scale=0.20]{figures/simulation/2020-05-28/beta12.pdf}
\includegraphics[scale=0.20]{figures/simulation/2020-05-28/beta22.pdf}
\includegraphics[scale=0.20]{figures/simulation/2020-05-28/beta32.pdf}
\includegraphics[scale=0.20]{figures/simulation/2020-05-28/beta42.pdf} 
\end{tabular}
\caption{Histogram plots of $\hat{\bbeta}_1$ and $\hat{\bbeta}_2$. Red lines indicate average and blue lines indicate true values.} \label{fig:betahat}
\end{figure}
The initial parameters for $\balpha$, $\bxi$, $\bsigma^2$ and $\bphi$ are simulated as follows:
\begin{align*}
\alpha_{ik} \sim \textup{Unif(-0.25,0.25), } \xi_k,\phi_i \sim \textup{Unif(0.01,0.04) and }
\sigma^2_i \sim \textup{Unif(0.4,0.6)}. 
\end{align*}
We consider a sequence of penalty parameters and common latent fields given by:
\begin{align*}
\boldsymbol{\lambda} = (100,80,60,40,20,10,4,2,1,0) \textup{ and } \boldsymbol{q}=(0,1,2),
\end{align*}
respectively. The algorithm is set to convergence, whenever $\left\vert \frac{l_-(\btheta^{(n+1)})-l_-(\btheta^{(n)})}{l_-(\btheta^{(n)})} \right\vert < 10^{-6}$.


\textcolor{red}{comment on CV}

\textcolor{red}{How does these results coincide with CV performance? Hopefully we see, that it is most likely that the minimal CV-score is when $\lambda=20$ and $q=2$.} 

The middle panel in Figure \ref{fig:cvrmse} show that $RMSE(\hat{\boldsymbol{A}})$ significantly decreases in average when the number of common latent fields increases. This emphasizes that when adding more latent fields to the model, it induces more flexibility to identify the dependency structure for the multivariate LGCP. For $q=1,2$ the penalized regression achieves a strict convex for the $RMSE(\hat{\boldsymbol{A}})$, where in average the minimal $RMSE(\hat{\boldsymbol{A}})$ is estimated from $q=2$ and $\lambda=20$. Moreover, smaller values of $\lambda$ increases the average of $RMSE(\hat{\boldsymbol{A}})$ substantially, which is mainly affected by outlier estimates caused by the identifiability issue described in Section \ref{sec:ident}. This emphasizes an another advantage of using penalized estimation of $\balpha$, since higher penalties constraints for numerical higher estimated values of $\balpha$ and thereby detain the outliers caused by the identifiability issue. In addition, when adding a strict convex penalty function to the convex conditional likelihood function it can even help to ensure that the estimation algorithm does not get stuck in a local minimum caused by the identifiability issue. 

Regarding the estimates of $\bsigma^2$, the right panel in Figure \ref{fig:cvrmse} show that $RMSE(\hat{\bsigma}^2)$ significantly descreases when $q$ increases. This is not surpricing since the estimates of $\bsigma^2$ depend on the estimates of $\balpha$. However, $\hat{\bsigma}^2$ are only mildly affected by $\lambda$. Notice that the estimates of $\bsigma^2$ for $q=0$ is simply overestimated due to $\hat{\balpha} = \boldsymbol{0}$, since the variance of $X_i$ also gets a contribution from $\sum_{k=1}^q \alpha_{ik}^2$. Thus the variance of $X_i$ gets overcompensated by the estimates of $\bsigma^2$. Moreover, for $q=2$ a slight increase in $RMSE(\hat{\bsigma}^2)$ as $\lambda$ increases  can maybe also be explained by overestimation of $\bsigma^2$ caused by large penalty on $\balpha$. 
\begin{figure}[ht!]
\centering
\begin{tabular}{c c c}
\includegraphics[scale=0.3]{figures/simulation/2020-06-05/cv_heatmap.pdf}
\includegraphics[scale=0.3]{figures/simulation/2020-06-05/conf_aa.pdf}
\includegraphics[scale=0.3]{figures/simulation/2020-06-05/conf_sig.pdf}
\end{tabular}
\caption{Left: Distribution of overall minimum CV-scores. Middle: Average of $RMSE(\hat{\boldsymbol{A}})$ for $\boldsymbol{q}$ and $\boldsymbol{\lambda}$. Right: Average of $RMSE(\hat{\bsigma}^2)$ for $\boldsymbol{q}$ and $\boldsymbol{\lambda}$.} \label{fig:cvrmse}
\end{figure}

\begin{figure}[ht!]
\begin{tabular}{c c c c}
\includegraphics[scale=0.21]{figures/simulation/2020-06-05/pcf_est_12.pdf}
\includegraphics[scale=0.21]{figures/simulation/2020-06-05/pcf_est_24.pdf}
\includegraphics[scale=0.21]{figures/simulation/2020-06-05/pcf_est_25.pdf}
\includegraphics[scale=0.21]{figures/simulation/2020-06-05/pcf_est_34.pdf} \\
\includegraphics[scale=0.21]{figures/simulation/2020-06-05/pcf_est_22.pdf}
\includegraphics[scale=0.21]{figures/simulation/2020-06-05/pcf_est_23.pdf}
\includegraphics[scale=0.21]{figures/simulation/2020-06-05/pcf_est_45.pdf}
\includegraphics[scale=0.21]{figures/simulation/2020-06-02/pcf_est_55.pdf}
\end{tabular}
\caption{Examples of estimates of PCF's or cross-PCF's (red lines) compared to the true PCF or true cross-PCF (blue line).} \label{fig:boxp}
\end{figure}

\begin{figure}[ht!]
\centering
\begin{tabular}{| c | c c c c c c c c c c c |}
\hline
 &0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
\hline
$\#$ Zeros & 30 & 43 & 16 & 7 & 1 & 3 & 0 & 0 & 0& 0 & 0\\
\hline
\end{tabular}
\end{figure}

\subsection{Five-variate Thomas process}

\textcolor{red}{What if the point processes is simulated from a multivariate Thomas process? Is the model still able to capture the dependence structure?}



==> setup/macros.tex <==

%  A simple AAU report template.
%  2014-09-13 v. 1.1.0
%  Copyright 2010-2014 by Jesper KjÃ¦r Nielsen <jkn@es.aau.dk>
%
%  This is free software: you can redistribute it and/or modify
%  it under the terms of the GNU General Public License as published by
%  the Free Software Foundation, either version 3 of the License, or
%  (at your option) any later version.
%
%  This is distributed in the hope that it will be useful,
%  but WITHOUT ANY WARRANTY; without even the implied warranty of
%  MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
%  GNU General Public License for more details.
%
%  You can find the GNU General Public License at <http://www.gnu.org/licenses/>.
%
%
%
% see, e.g., http://en.wikibooks.org/wiki/LaTeX/Customizing_LaTeX#New_commands
% for more information on how to create macros

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros for the titlepage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Creates the aau titlepage
\newcommand{\aautitlepage}[3]{%
  {
    %set up various length
    \ifx\titlepageleftcolumnwidth\undefined
      \newlength{\titlepageleftcolumnwidth}
      \newlength{\titlepagerightcolumnwidth}
    \fi
    \setlength{\titlepageleftcolumnwidth}{0.5\textwidth-\tabcolsep}
    \setlength{\titlepagerightcolumnwidth}{\textwidth-3\tabcolsep-\titlepageleftcolumnwidth}
    %create title page
    \thispagestyle{empty}
    \noindent%
    \begin{tabular}{@{}ll@{}}
      \parbox{\titlepageleftcolumnwidth}{
        \iflanguage{danish}{%
          \includegraphics[width=\titlepageleftcolumnwidth]{figures/aau_logo_da}
        }{%
          \includegraphics[width=\titlepageleftcolumnwidth]{figures/aau_logo_en}
        }
      } &
      \parbox{\titlepagerightcolumnwidth}{\raggedleft\sf\small
        #2
      }\bigskip\\
       #1 &
      \parbox[t]{\titlepagerightcolumnwidth}{%
      \textbf{Abstract:}\bigskip\par
        \fbox{\parbox{\titlepagerightcolumnwidth-2\fboxsep-2\fboxrule}{%
          #3
        }}
      }\\
    \end{tabular}
    \vfill
    \iflanguage{danish}{%
      \noindent{\footnotesize\emph{Rapportens indhold er frit tilgængeligt, men offentliggørelse (med kildeangivelse) må kun ske efter aftale med forfatterne.}}
    }{%
      \noindent{\footnotesize\emph{The content of this report is freely available, but publication (with reference) may only be pursued due to agreement with the author.}}
    }
    \clearpage
  }
}

%Create english project info
\newcommand{\englishprojectinfo}[8]{%
  \parbox[t]{\titlepageleftcolumnwidth}{
    \textbf{Title:}\\ #1\bigskip\par
    \textbf{Theme:}\\ #2\bigskip\par
    \textbf{Project Period:}\\ #3\bigskip\par
    \textbf{Project Group:}\\ #4\bigskip\par
    \textbf{Participants:}\\ #5\bigskip\par
    \textbf{Supervisor:}\\ #6\bigskip\par
    \textbf{Copies:} #7\bigskip\par
    \textbf{Page Numbers: }\pageref{LastPage}  \bigskip\par
    \textbf{Date of Completion:}\\ #8
  }
}

%Create danish project info
\newcommand{\danishprojectinfo}[8]{%
  \parbox[t]{\titlepageleftcolumnwidth}{
    \textbf{Titel:}\\ #1\bigskip\par
    \textbf{Tema:}\\ #2\bigskip\par
    \textbf{Projektperiode:}\\ #3\bigskip\par
    \textbf{Projektgruppe:}\\ #4\bigskip\par
    \textbf{Deltager:}\\ #5\bigskip\par
    \textbf{Vejleder:}\\ #6\bigskip\par
    \textbf{Oplagstal:} #7\bigskip\par
    \textbf{Sidetal:} \pageref{LastPage}  \bigskip\par
    \textbf{Afleveringsdato:}\\ #8
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% An example environment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremheaderfont{\normalfont\bfseries}
\theorembodyfont{\normalfont}
\theoremstyle{break}
\def\theoremframecommand{{\color{aaublue!50}\vrule width 5pt \hspace{5pt}}}


\newshadedtheorem{sat}{Theorem}[section]
\newenvironment{satning}{%
		\begin{sat}
}{%
		\end{sat}
}


\newshadedtheorem{prop}[sat]{Proposition}
\newenvironment{proposition}{%
		\begin{prop}
}{%
		\end{prop}
}

\newshadedtheorem{lem}[sat]{Lemma}
\newenvironment{lemma}{%
		\begin{lem}
}{%
		\end{lem}
}

\newshadedtheorem{mydef}[sat]{Definition}
\newenvironment{definition}[1]{%
		\begin{mydef}[#1]
}{%
		\end{mydef}
}

\newenvironment{Korollar}[1]{%
		\begin{cor}[#1]
}{%
		\end{cor}
}



\newshadedtheorem{cor}[sat]{Korollar}

\theoremstyle{break}
\theoremsymbol{\ensuremath{\blacksquare}}
\newtheorem*{bevis}{Proof}
\theoremsymbol{\ensuremath{\square}}

\newtheorem{eks}[sat]{Eksempel}
\newenvironment{Eksempel}{%
		\begin{eks}
}{%
		\end{eks}
}

\newtheorem{bem}[sat]{Remark}
\newenvironment{Bemarkning}{%
		\begin{bem}
}{%
		\end{bem}
}

\renewcommand{\qedsymbol}{}

\setlength{\delimitershortfall}{0pt} %SÃ¸rger for at matrix med partial diff lukker helt til i toppen

%smÃ¥ bogstaver med fed
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\bee}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bm}{\mathbf{m}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bttt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
%store bogstaver med fed
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bTT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

%SmÃ¥ bogstaver med tilde og fed
\newcommand{\tba}{\widetilde{\mathbf{a}}}
\newcommand{\tbb}{\widetilde{\mathbf{b}}}
\newcommand{\tbc}{\widetilde{\mathbf{c}}}
\newcommand{\tbd}{\widetilde{\mathbf{d}}}
\newcommand{\tbe}{\widetilde{\mathbf{e}}}
\newcommand{\tbf}{\widetilde{\mathbf{f}}}
\newcommand{\tbg}{\widetilde{\mathbf{g}}}
\newcommand{\tbh}{\widetilde{\mathbf{h}}}
\newcommand{\tbi}{\widetilde{\mathbf{i}}}
\newcommand{\tbj}{\widetilde{\mathbf{j}}}
\newcommand{\tbk}{\widetilde{\mathbf{k}}}
\newcommand{\tbl}{\widetilde{\mathbf{l}}}
\newcommand{\tbm}{\widetilde{\mathbf{m}}}
\newcommand{\tbn}{\widetilde{\mathbf{n}}}
\newcommand{\tbo}{\widetilde{\mathbf{o}}}
\newcommand{\tbp}{\widetilde{\mathbf{p}}}
\newcommand{\tbq}{\widetilde{\mathbf{q}}}
\newcommand{\tbr}{\widetilde{\mathbf{r}}}
\newcommand{\tbs}{\widetilde{\mathbf{s}}}
\newcommand{\tbt}{\widetilde{\mathbf{t}}}
\newcommand{\tbu}{\widetilde{\mathbf{u}}}
\newcommand{\tbv}{\widetilde{\mathbf{v}}}
\newcommand{\tbw}{\widetilde{\mathbf{w}}}
\newcommand{\tbx}{\widetilde{\mathbf{x}}}
\newcommand{\tby}{\widetilde{\mathbf{y}}}
\newcommand{\tbz}{\widetilde{\mathbf{z}}}

%SmÃ¥ bogstaver med hat
\newcommand{\ha}{\widehat{a}}
\newcommand{\hb}{\widehat{b}}
\newcommand{\hc}{\widehat{c}}
\newcommand{\hd}{\widehat{d}}
\newcommand{\he}{\widehat{e}}
\newcommand{\hf}{\widehat{f}}
\newcommand{\hg}{\widehat{g}}
\newcommand{\hh}{\widehat{h}}
\newcommand{\hi}{\widehat{i}}
\newcommand{\hj}{\widehat{j}}
\newcommand{\hk}{\widehat{k}}
\newcommand{\hl}{\widehat{l}}
\newcommand{\hm}{\widehat{m}}
\newcommand{\hn}{\widehat{n}}
\newcommand{\ho}{\widehat{o}}
\newcommand{\hp}{\widehat{p}}
\newcommand{\hq}{\widehat{q}}
\newcommand{\hr}{\widehat{r}}
\newcommand{\hs}{\widehat{s}}
\newcommand{\htt}{\widehat{t}}
\newcommand{\hu}{\widehat{u}}
\newcommand{\hv}{\widehat{v}}
\newcommand{\hw}{\widehat{w}}
\newcommand{\hx}{\widehat{x}}
\newcommand{\hy}{\widehat{y}}
\newcommand{\hz}{\widehat{z}}

%SmÃ¥ bogstaver med tilde
\newcommand{\ta}{\widetilde{a}}
\newcommand{\tb}{\widetilde{b}}
\newcommand{\tc}{\widetilde{c}}
\newcommand{\td}{\widetilde{d}}
\newcommand{\te}{\widetilde{e}}
\newcommand{\tf}{\widetilde{f}}
\newcommand{\tg}{\widetilde{g}}
\newcommand{\thh}{\widetilde{h}}
\newcommand{\ti}{\widetilde{i}}
\newcommand{\tj}{\widetilde{j}}
\newcommand{\tk}{\widetilde{k}}
\newcommand{\tl}{\widetilde{l}}
\newcommand{\tm}{\widetilde{m}}
\newcommand{\tn}{\widetilde{n}}
\newcommand{\tooo}{\widetilde{o}}
\newcommand{\tp}{\widetilde{p}}
\newcommand{\tq}{\widetilde{q}}
\newcommand{\trr}{\widetilde{r}}
\newcommand{\ts}{\widetilde{s}}
\newcommand{\ttt}{\widetilde{t}}
\newcommand{\tu}{\widetilde{u}}
\newcommand{\tv}{\widetilde{v}}
\newcommand{\tw}{\widetilde{w}}
\newcommand{\tx}{\widetilde{x}}
\newcommand{\ty}{\widetilde{y}}
\newcommand{\tz}{\widetilde{z}}

%SmÃ¥ bogstaver med fed og overline
\newcommand{\obs}{\overline{\mathbf{s}}}

%Store bogstaver med tilde og fed
\newcommand{\tbA}{\widetilde{\mathbf{A}}}
\newcommand{\tbB}{\widetilde{\mathbf{B}}}
\newcommand{\tbC}{\widetilde{\mathbf{C}}}
\newcommand{\tbD}{\widetilde{\mathbf{D}}}
\newcommand{\tbE}{\widetilde{\mathbf{E}}}
\newcommand{\tbF}{\widetilde{\mathbf{F}}}
\newcommand{\tbG}{\widetilde{\mathbf{G}}}
\newcommand{\tbH}{\widetilde{\mathbf{H}}}
\newcommand{\tbI}{\widetilde{\mathbf{I}}}
\newcommand{\tbJ}{\widetilde{\mathbf{J}}}
\newcommand{\tbK}{\widetilde{\mathbf{K}}}
\newcommand{\tbL}{\widetilde{\mathbf{L}}}
\newcommand{\tbM}{\widetilde{\mathbf{M}}}
\newcommand{\tbN}{\widetilde{\mathbf{N}}}
\newcommand{\tbO}{\widetilde{\mathbf{O}}}
\newcommand{\tbP}{\widetilde{\mathbf{P}}}
\newcommand{\tbQ}{\widetilde{\mathbf{Q}}}
\newcommand{\tbR}{\widetilde{\mathbf{R}}}
\newcommand{\tbS}{\widetilde{\mathbf{S}}}
\newcommand{\tbT}{\widetilde{\mathbf{T}}}
\newcommand{\tbU}{\widetilde{\mathbf{U}}}
\newcommand{\tbV}{\widetilde{\mathbf{V}}}
\newcommand{\tbW}{\widetilde{\mathbf{W}}}
\newcommand{\tbX}{\widetilde{\mathbf{X}}}
\newcommand{\tbY}{\widetilde{\mathbf{Y}}}
\newcommand{\btZ}{\widetilde{\mathbf{Z}}}
\newcommand{\tbZ}{\widetilde{\mathbf{Z}}}


%Fede tal
\newcommand{\bnul}{\mathbf{0}}
\newcommand{\bet}{\mathbf{1}}
\newcommand{\bto}{\mathbf{2}}
\newcommand{\btre}{\mathbf{3}}
\newcommand{\bfire}{\mathbf{4}}
\newcommand{\bfem}{\mathbf{5}}
\newcommand{\bseks}{\mathbf{6}}
\newcommand{\bsyv}{\mathbf{7}}
\newcommand{\botte}{\mathbf{8}}
\newcommand{\bni}{\mathbf{9}}
%black board bold bogstaver
\newcommand{\A}{\mathbb{A}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\Rn}{\mathbb{R}^n}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}

%Mathcal bogstaver
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%Hat bogstaver
\newcommand{\hcK}{\widehat{\cK}}
\newcommand{\hK}{\widehat{K}}
\newcommand{\hL}{\widehat{L}}
\newcommand{\hF}{\widehat{F}}
\newcommand{\hG}{\widehat{G}}
\newcommand{\hJ}{\widehat{J}}

%Mathscr
\newcommand{\sA}{\mathscr{A}}
\newcommand{\sB}{\mathscr{B}}
\newcommand{\sC}{\mathscr{C}}
\newcommand{\sD}{\mathscr{D}}
\newcommand{\sE}{\mathscr{E}}
\newcommand{\sF}{\mathscr{F}}
\newcommand{\sG}{\mathscr{G}}
\newcommand{\sH}{\mathscr{H}}
\newcommand{\sI}{\mathscr{I}}
\newcommand{\sJ}{\mathscr{J}}
\newcommand{\sK}{\mathscr{K}}
\newcommand{\sL}{\mathscr{L}}
\newcommand{\sM}{\mathscr{M}}
\newcommand{\sN}{\mathscr{N}}
\newcommand{\sO}{\mathscr{O}}
\newcommand{\sP}{\mathscr{P}}
\newcommand{\sQ}{\mathscr{Q}}
\newcommand{\sR}{\mathscr{R}}
\newcommand{\sS}{\mathscr{S}}
\newcommand{\sT}{\mathscr{T}}
\newcommand{\sU}{\mathscr{U}}
\newcommand{\sV}{\mathscr{V}}
\newcommand{\sW}{\mathscr{W}}
\newcommand{\sX}{\mathscr{X}}
\newcommand{\sY}{\mathscr{Y}}
\newcommand{\sZ}{\mathscr{Z}}


%Store grÃ¦ske bogstaver
\newcommand{\bT}{\Theta}

%GrÃ¦ske bogstaver med fed
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bphi}{\boldsymbol{\varphi}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\be}{\boldsymbol{\varepsilon}}
\newcommand{\bepsilon}{\boldsymbol{\varepsilon}}

%SmÃ¥ grÃ¦ske bogstaver med hat
\newcommand{\gh}{\widehat{\gamma}}
\newcommand{\sh}{\widehat{\sigma}}
\newcommand{\rh}{\widehat{\rho}}
\newcommand{\hgamma}{\widehat{\gamma}}
\newcommand{\hsigma}{\widehat{\sigma}}
\newcommand{\hrho}{\widehat{\rho}}
\newcommand{\hbeta}{\widehat{\beta}}
\newcommand{\hepsilon}{\widehat{\varepsilon}}
\newcommand{\halpha}{\widehat{\alpha}}


%Store grÃ¦ske bogstaver med hat
\newcommand{\Gh}{\widehat{\Gamma}}
\newcommand{\Rh}{\widehat{R}}
\newcommand{\hGamma}{\widehat{\Gamma}}
\newcommand{\hRho}{\widehat{R}}

%Store grÃ¦ske bogstaver med tilde
\newcommand{\tAlpha}{\widetilde{A}}
\newcommand{\tBeta}{\widetilde{B}}
\newcommand{\tGamma}{\widetilde{\Gamma}}
\newcommand{\tDelta}{\widetilde{\Delta}}
\newcommand{\tEpsilon}{\widetilde{\E}}
\newcommand{\tOmega}{\widetilde{\Omega}}

%GrÃ¦ske bogstaver med tilde og fed
\newcommand{\tbmu}{\widetilde{\boldsymbol{\mu}}}
\newcommand{\btt}{\boldsymbol{\widetilde{\theta}}}


%GrÃ¦ske bogstaver med fed og overline
\newcommand{\obphi}{\overline{\boldsymbol{\phi}}}


%Store grÃ¦ske bogstaver med tilde og fed

%GrÃ¦ske bogstaver med hat og fed
\newcommand{\bth}{\boldsymbol{\widehat{\theta}}}
\newcommand{\hbtheta}{\widehat{\boldsymbol{\theta}}}
\newcommand{\bbh}{\widehat{\boldsymbol{\beta}}}
\newcommand{\hbbeta}{\widehat{\boldsymbol{\beta}}}
\newcommand{\bsh}{\widehat{\boldsymbol{\sigma}}}
\newcommand{\hbsigma}{\widehat{\boldsymbol{\sigma}}}
\newcommand{\brh}{\widehat{\boldsymbol{\rho}}}
\newcommand{\hbrho}{\widehat{\boldsymbol{\rho}}}
\newcommand{\bgh}{\widehat{\boldsymbol{\gamma}}}
\newcommand{\hbgamma}{\widehat{\boldsymbol{\gamma}}}
\newcommand{\bmh}{\widehat{\boldsymbol{\mu}}}
\newcommand{\hbmu}{\widehat{\boldsymbol{\mu}}}
\newcommand{\bphih}{\widehat{\boldsymbol{\varphi}}}
\newcommand{\hbphi}{\widehat{\boldsymbol{\varphi}}}

%Store grÃ¦ske bogstaver med hat og fed

%GrÃ¦ske bogstaver med hat og tilde
\newcommand{\sht}{\widetilde{\widehat{\sigma}}}
%Ting der skal redefineres
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\phi}{\varphi}
\renewcommand{\Re}{\textup{Re}}

%Textup kommandoer
\newcommand{\E}{\textup{E}}
\newcommand{\Var}{\textup{Var}}
\newcommand{\Cov}{\textup{Cov}}
\newcommand{\bspan}{\textup{span}}
\newcommand{\rank}{\textup{rank}}
\newcommand{\range}{\textup{range}}
\newcommand{\AIC}{\textup{AIC}}


%Ting i declareMathOperator
\DeclareMathOperator*{\slim}{s-lim}
\DeclareMathOperator*{\flim}{f-lim}
\DeclareMathOperator*{\inte}{int}
\DeclareMathOperator*{\epi}{epi}
\DeclareMathOperator*{\GL}{GL_n(\mathbb{R})}
\DeclareMathOperator*{\SL}{SL_n(\mathbb{R})}\DeclareMathOperator*{\On}{O_n(\mathbb{R})}\DeclareMathOperator*{\SON
}{SO_n(\mathbb{R})}
\DeclareMathOperator*{\Ker}{Ker}
\DeclareMathOperator*{\so}{SO_2(\mathbb{R})}
\DeclareMathOperator*{\oo}{O_2(\mathbb{R})}
\DeclareMathOperator*{\Isom}{Isom(\mathbb{R}^2)}
\DeclareMathOperator*{\Sym}{Sym}
\DeclareMathOperator*{\tr}{tr}
\DeclareMathOperator*{\gl}{GL_2(\mathbb{Z})}

\DeclareMathOperator*{\Col}{Col}
%\DeclareMathOperator*{\Var}{Var}
\DeclareMathOperator*{\Int}{Int}
%\DeclareMathOperator*{\Cov}{Cov}
\DeclareMathOperator*{\Corr}{Corr}




\newcommand{\id}{\mathrm{id}}

\newcommand{\tal}{\setcounter{section}{1}
\setcounter{sat}{0}}


\newcommand{\bbt}{\bar{\boldsymbol{\theta}}}

\newcommand{\bhx}{\widehat{\mathbf{x}}}
\newcommand{\btx}{\widetilde{\mathbf{x}}}


\newcommand{\pdif}[1]{\frac{\partial}{\partial#1} }

\newcommand{\abs}[1]{\vert #1 \vert}
\newcommand{\nor}[1]{\Vert #1 \Vert}
\newcommand{\lr}[1]{\langle #1 \rangle}


